Certificates for triangular equivalence and rank profiles

In this paper, we give novel certificates for triangular equivalence and rank profiles. These certificates enable to verify the row or column rank profiles or the whole rank profile matrix faster than recomputing them, with a negligible overall overhead. We first provide quadratic time and space non-interactive certificates saving the logarithmic factors of previously known ones. Then we propose interactive certificates for the same problems whose Monte Carlo verification complexity requires a small constant number of matrix-vector multiplications, a linear space, and a linear number of extra field operations. As an application we also give an interactive protocol, certifying the determinant of dense matrices, faster than the best previously known one.

==> mulmuley.tex <==
\section*{Alternative using geometric progression
  vectors}\label{sec:geom}
\subsection*{Representative Laurent polynomial of a matrix}

If a matrix is lower triangular, then 
$\begin{bmatrix}1&X&X^2&\ldots&X^{n-1}\end{bmatrix}\cdot{}L\cdot\begin{bmatrix}1\\X^{-1}\\\vdots\\X^{1-n}\end{bmatrix}$
is a polynomial in $X$.

\begin{algorithm}[htb]
  \caption{Representative Laurent polynomial $P_{A}(X)$}\label{alg:alldiag}
  \begin{algorithmic}[1]
    \REQUIRE $A \in \F^{m{\times}n}$.    
    \ENSURE $P_A\in \F(X)$.
    \FOR{$k=1-m$ \TO $n-1$}
      \STATE $p_k=0$
      \FOR{$i=1$ \TO $m$}
        \IF{$i>k$ \AND $i-k{\leq}n$}
          \STATE $p_k += A_{i;i-k}$
        \ENDIF
      \ENDFOR
    \ENDFOR
    \RETURN $P_A(X)=\sum_{k=1-m}^{n-1}p_k X^k$.
  \end{algorithmic}
\end{algorithm}

\subsection*{Constant round triangular equivalence certificate}

\newlength{\arrowlength}
\settowidth{\arrowlength}{\scriptsize$1000$}
\newcommand{\fxrightarrow}[1]{\xrightarrow{\mathmakebox[\arrowlength]{#1}}}
\newcommand{\fxleftarrow}[1]{\xleftarrow{\mathmakebox[\arrowlength]{#1}}}

\begin{figure*}[htbp]
  \centering
  \begin{tabular}{|c c l|}
    \hline\rule{0pt}{12pt}   
    Prover &  & Verifier \\
    & $ A, B \in \mathbb{F}^{m{\times}n} $ &  \\
    & $A$ is regular, $m{\geq}n$ & \\
    \hdashline\rule{0pt}{12pt}
\\[-12pt]
    $L$ lower triang. s.t. $AL= B$ & $\fxrightarrow{\exists{}L}$ & \\
    \hdashline\rule{0pt}{12pt}   
\\[-12pt]
    & $\fxleftarrow{D}$& $D\sample{DiagonalMatrix}$ \\
    $g(X)=P_{LD}(X)$      & $\fxrightarrow{g(X)}$& $g\stackrel{?}{\in}\F_{n-1}[X]$ \\
    & $\fxleftarrow{r}$& $r\sample{\F}$ \\
    $z$, s.t. $\begin{bmatrix}1&r&\ldots&r^{n-1}\end{bmatrix}=z^T\cdot{}A$      
    & $\fxrightarrow{z}$
    & $z^T\cdot{}A\checks{==}\begin{bmatrix}1&r&\ldots&r^{n-1}\end{bmatrix}$ \\
    && $z^T\cdot{}B\cdot{}D\cdot\begin{bmatrix}1\\r^{-1}\\\vdots\\r^{1-n}\end{bmatrix}\checks{==}g(r)$ \\
    \hline
  \end{tabular}
  \caption{Constant round linear communication certificate for triangular equivalence}
  \label{cert:treqpol}
\end{figure*}

\begin{theorem} Certificate~\ref{cert:treqpol} is perfectly complete
  and sound.
\end{theorem}
\begin{proof}
Correctness: 
\begin{multline}
z^T\cdot{}B\cdot{}D\cdot\begin{bmatrix}1\\r^{-1}\\\vdots\\r^{1-n}\end{bmatrix}=
z^T\cdot{}A\cdot{}L\cdot{}D\cdot\begin{bmatrix}1\\r^{-1}\\\vdots\\r^{1-n}\end{bmatrix}=\\
\begin{bmatrix}1&r&\ldots&r^{n-1}\end{bmatrix}\cdot{}L\cdot{}D\cdot\begin{bmatrix}1\\r^{-1}\\\vdots\\r^{1-n}\end{bmatrix}=P_{L\cdot{}D}(r)
\end{multline}

Soundess:
\begin{itemize}
\item
  $z^T\cdot{}A\checks{==}\begin{bmatrix}1&r&\ldots&r^{1-n}\end{bmatrix}$
  is deterministic.
\item if $L$ is not triangular then its upper part is not identically
  zero. Therefore by considering $D$ as a diagonal matrix of
  indeterminates at least one coefficient of negative degree of the
  representative rational fraction $DL$ will be non identically zero.
  As those are of degree $1$ in the indeterminates of $D$, for a
  random diagonal $D$, the representative rational fraction of $DL$
  will not be a polynomial with probability at least $1-\frac{1}{q}$.
\item if $g$ is not a polynomial of degree at most $n-1$, it is not the
  representative of a triangular matrix.
\item if $g$ is not the representative polynomial of
  $DL$ then by Zippel-Schwartz, its evaluation at $r$ will fail with
  probability $1-2\frac{n-1}{q}$ (since $X^{n-1}(g-g_{DL})(X)$ is a
  polynomial of degree at most $2(n-1)$).
\end{itemize}
\end{proof}

\TODO{Workout probabilities if
  $D=diag(1,\lambda,\ldots,\lambda^{n-1})$, so that the number of
  random samples is $O(1)$ ... }
\ \\

\TODO{Produce a constant round certificate for Generic Rank
  Profileness ...}


%\begin{figure*}[htbp]
%  \centering
%  \begin{tabular}{|c c l|}
%    \hline\rule{0pt}{12pt}   
%    Prover &  & Verifier \\
%    & $ A \in \mathbb{F}^{m{\times}n} $ &  \\
%    \hdashline\rule{0pt}{12pt}
%    $A=LRU$  & $\fxrightarrow{R}$& \\
%    \hdashline\rule{0pt}{12pt}   
%    & $\fxleftarrow{D_1}$& $D_1\sample{\F^m}$ \\
%    $g(X)=P_{D_1L}(X)$      & $\fxrightarrow{g(X)}$& $g\stackrel{?}{\in}\F_{m-1}[X]$ \\
%    & $\fxleftarrow{D_2}$& $D_2\sample{\F^n}$ \\
%    $h(X)=P_{UD_2}(X)$      & $\fxrightarrow{h(X)}$& $h\stackrel{?}{\in}\F_{n-1}[X]$ \\
%    \hdashline\rule{0pt}{12pt}   
%    & $\fxleftarrow{r_1,r_2}$& $r_1,r_2\sample{\F}$ \\
%    $z^T=\begin{bmatrix}r_1&r_1^2&\ldots&r_1^m\end{bmatrix}D_1L$      
%    & $\fxrightarrow{z}$
%    & $z^T\cdot{}\begin{bmatrix}r_1^{-1}\\\vdots\\r_1^{-m}\end{bmatrix}\checks{==}g(r_1)$ \\
%    $x=UD_2\begin{bmatrix}r_2\\\vdots\\r_2^n\end{bmatrix}$      
%    & $\fxrightarrow{x}$
%    & $\begin{bmatrix}r_2^{-1}&\ldots&r_2^{-n}\end{bmatrix}\cdot{}x\checks{==}h(r_2)$ \\
%    \hdashline\rule{0pt}{12pt}   
%    && $z^T\cdot{}R\cdot{}x\checks{==}\begin{bmatrix}r_1&\ldots&r_1^{m}\end{bmatrix}D_1AD_2\begin{bmatrix}r_2\\\vdots\\r_2^n\end{bmatrix}$ \\
%    \hline
%  \end{tabular}
%  \caption{Linear communication certificate for the rank profile matrix}
%  \label{cert:rpmpol}
%\end{figure*}


%\begin{theorem}
%\end{theorem}
%\begin{proof}

%Soundess: If $A \neq LRU$, then 
%$\begin{bmatrix}r_1&\ldots&r_1^{m}\end{bmatrix}D_1(A-LRU)D_2\begin{bmatrix}r_2\\\vdots\\r_2^n\end{bmatrix}$
%is non zero with probability less than $1-\frac{m+n}{q}$ by Freivalds,

%\TODO{In fact as is, the certificate shows that there exists $L^*$ and
%  $U^*$ such that $A=L^*RU^*$ w.h.p. but the guaranty is only that
%  $L^*$ and $U^*$ have their upper (resp. lower) diagonals that sum to
%  $0$ ...}
%\end{proof}

